Exploring Factors and Metrics to Select Open Source Software Components for Integration: An Empirical Study

[Context] Open Source Software (OSS) is nowadays used and integrated in most of the commercial products. However, the selection of OSS projects for integration is not a simple process, mainly due to a of lack of clear selection models and lack of information from the OSS portals. [Objective] We investigate the factors and metrics that practitioners currently consider when selecting OSS. We also investigate the source of information and portals that can be used to assess the factors, as well as the possibility to automatically extract such information with APIs. [Method] We elicited the factors and the metrics adopted to assess and compare OSS performing a survey among 23 experienced developers who often integrate OSS in the software they develop. Moreover, we investigated the APIs of the portals adopted to assess OSS extracting information for the most starred 100K projects in GitHub. [Result] We identified a set consisting of 8 main factors and 74 sub-factors, together with 170 related metrics that companies can use to select OSS to be integrated in their software projects. Unexpectedly, only a small part of the factors can be evaluated automatically, and out of 170 metrics, only 40 are available, of which only 22 returned information for all the 100K projects. Therefore, we recommend project maintainers and project repositories to pay attention to provide information for the project they are hosting, so as to increase the likelihood of being adopted [Conclusion] OSS selection can be partially automated, by extracting the information needed for the selection from portal APIs. OSS producers can benefit from our results by checking if they are providing all the information commonly required by potential adopters...

==> Figures/examples/client-js.tex <==
const $app = document.getElementById('app');

function renderPage() {
  $app.innerHTML = `
    <h1 id="heading">The Micro-Frontend</h1>
    <team-catalog id="catalog"></team-catalog>
    <team-actions id="actions"></team-actions>
  `;
}


==> Figures/examples/server-side-config.tex <==
upstream catalog {
  server team_catalog:8081;
}
upstream actions {
  server team_actions:8082;
}

server {
  listen 8080;
  ssi on;

  location /catalog {
    proxy_pass  http://team_catalog;
  }
  location /actions {
    proxy_pass  http://team_actions;
  }
  location /shell {
    proxy_pass  http://team_shell;
  }
  location / {
    proxy_pass  http://team_shell;
  }
}

==> Sections/4_Results.tex <==
% The sample of interviewees was not determined in advance. A preplanned sample would have allowed for a more controlled result analysis, but it would also have limited the possibility to add interviewees to the set in an unanticipated manner. We are fully aware that this may have somewhat influenced our results.
Here we first provide information about the sample of respondents, which can be used to better interpret the results and then, we show the collected results with a concise analysis of the responses obtained, with insights gained by statistical analysis.


We collected 23 interviews from experienced practitioners. 
Figure~\ref{img:sizes} contains the distribution of company sizes where our interviewees belong, while Figure~\ref{img:roles} shows the percentage for organizational roles identified in the questionnaire.


% The first immediate result is that, compared to our previous survey [6], several new factors have been identified while others are not considered. Unexpectedly, most of the development factors, license issues, and quality aspects such as complexity, performance and usability are not considered as good factors for FLOSS adoption.
% However, since several factors identified in this first round of interviews are pretty similar, the identification of similarities and difference will be analyzed after the results of the focus group.


% \todo[inline]{add a piechart to the right side of the tables}

  
% \begin{minipage}{\textwidth}
% \scriptsize
%   \begin{minipage}[]{0.49\textwidth}
%     \centering
% \begin{tabular}[c]{|l|l|} \hline
%         Company Size       & \# Interviewees \\ \hline
%         0-50               & 3             \\
%         50-250             & 2             \\
%         250-1000           & 7             \\
%         \textgreater{}1000 & 9            \\ \hline
%     \end{tabular}
    
%       \captionof{table}{A table beside a figure}
%       \label{tab:company-size}
%     \end{minipage}
%       \hfill
%     \begin{minipage}[c]{0.49\textwidth}
%     \centerline{\includegraphics[width=0.5\textwidth]{Figures/interviews_companysize.png}}
%     \captionof{figure}{Company size}
%     \label{img:companyPie}
%   \end{minipage}
% % \end{minipage}
% \vspace{2.5cm}
%   \begin{minipage}[c]{0.49\textwidth}
%      \centering

%   \begin{tabular}[c]{|l|l|} \hline
% Roles              & \# Interviewees  \\ \hline
% SW developer       & 8 \\
% Product Manager    & 7 \\
% Software Architect & 6 \\ \hline
% \end{tabular}
%       \captionof{table}{A table beside a figure}
%         \label{tab:tab-roles}
%     \end{minipage}
% \hfill
%     \begin{minipage}[c]{0.49\textwidth}
%     \centerline{\includegraphics[width=0.5\textwidth]{Figures/interviews_roles.png}}
%     \captionof{figure}{roles}
%     \label{img:rolesPie}
%   \end{minipage}
% \end{minipage}

\begin{figure}[t]
\centering
\subcaptionbox{}
{\begin{tabular}[c]{|p{2.5cm}|l|} 
         \hline
        Company Size (\# Employees)       & \# Interviewees \\ 
        \hline
        0-50               & 4             \\
        50-250             & 3             \\
        250-1000           & 7             \\
        \textgreater{}1000 & 9            \\ 
        \hline
      \end{tabular} }
\subcaptionbox{Distribution of company size}
{\includegraphics[width=0.4\linewidth,valign=b]{Figures/interviews_companysize.png}}
\caption{Distribution of company sizes of our interviewees}
\label{img:sizes}
\end{figure}
\begin{figure}[t]
\centering
\subcaptionbox{}
{\begin{tabular}[c]{|l|l|} \hline
        Roles              & \# Interviewees  \\ \hline
        SW developer       & 9 \\
        Product Manager    & 8 \\
        Software Architect & 6 \\ \hline
        \end{tabular}}
\subcaptionbox{The roles of our interviewees}
{\includegraphics[width=0.4\linewidth,valign=b]{Figures/interviews_roles.png}}
\caption{Figure caption}
\label{img:roles}
\end{figure}




\subsection{RQ1: Factors considered by practitioners when selecting OSS}
%table with list of factors, importance, metric adopted, sources



Our interviewees consider 8 main factors and 46 sub-factors when they select OSS, reporting an average of 2.35 factors per interviewee, a minimum of 1 and a maximum of 21 factors.
% \todo[inline]{we could add here: These factors and sub-factors can be found in the list identified in our Euromicro/SEAA systematic literature review \cite{Lenarduzzi2020SEAA}. However, it is worth noting that some factors became less important and were not mentioned by the interviewees. (btw, we could also calculate the no. of sub-factors in our questionnaire and show the percentage of sub-factors mentioned by the interviewees.)}

The factor that is mentioned more frequently from the interviewees is \textit{License} which has received a median importance of 4 out of 5. Surprisingly, this is not the value which has received the highest median value of importance as \textit{Community Support and Adoption, Performances} and \textit{Perceived Risk} received a median value of importance of 4.5 out of 5. 
It is interesting to note that no participant mentioned \textit{Economic}\rs{ and its } related \rs{sub-}factors such as license costs, or cost for training. 

In Table~\ref{tab:interviewees-portals-factors}, we report the list of factors and sub-factors together with the number of participants who mentioned them (column RQ1- \#) and the median of the importance reported by the interviewees (column RQ1 - Median).

% \begin{table}[H]
% \caption{High-level Factors considered during the adoption of OSS}
% \label{tab:interviewees-portals-factors}
% \centering
% \scriptsize
% % \begin{tabular}{p{2.5cm}|p{1.1cm}|p{1.5cm}|p{4cm}|}
% \begin{tabular}{|llp{0.1cm}|l|l|} \hline

% \multicolumn{4}{|l}{	\textbf{RQ1}	} &		&	\\ \hline

% \multicolumn{2}{|l}{	\textbf{Factor}	} &		&	\#	&	\textbf{Median}	\\ \hline
% \multicolumn{2}{|l}{	Community Support and Adoption	}		&		&	10	&	4.5	\\
% 		&	Popularity	&		&	9	&	3	\\
% 		&	Community reputation	&		&	11	&	3	\\
% 		&	Community size	&		&	13	&	3	\\
% 		&	Communication	&		&	6	&	3.5	\\
% 		&	Sustainability	&		&	11	&	3	\\
% 		&	Product Team	&		&	5	&	3	\\
% 		&	Fast response to bugs and faults	&		&	9	&	2	\\
% \multicolumn{2}{|l}{	Availability of Documentation	}		&		&	14	&	4	\\
% 		&	Availability of documentation/books/online docs	&		&	5	&	3	\\
% 		&	Software requirements	&		&	11	&	3	\\
% 		&	Hardware requirements	&		&	8	&	3.5	\\
% 		&	Road map	&		&	7	&	3	\\
% 		&	Test case documentation	&		&	4	&	3	\\
% 		&	Quality report	&		&	5	&	3	\\
% 		&	Coding comments	&		&	5	&	3	\\
% \multicolumn{2}{|l}{	License	}		&		&	21	&	4	\\
% \multicolumn{2}{|l}{	Operational SW Characteristics	}		&		&	6	&	4	\\
% 		&	Trialability	&		&	5	&	3	\\
% 		&	Independence from other SW	&		&	11	&	3	\\
% 		&	Development language	&		&	5	&	4	\\
% 		&	Multiplatform support	&		&	5	&	3	\\
% 		&	Standard compliance	&		&	5	&	4	\\
% \multicolumn{2}{|l}{	Maturity	}		&		&	6	&	3.5	\\

% \multicolumn{2}{|l}{	Quality	}		&		&	6	&	3.5	\\
% 		&	Reliability	&		&	3	&	4	\\
% 		&	Performances	&		&	4	&	4.5	\\
% 		&	Security 	&		&	15	&	4	\\
% 		&	Modularity	&		&	3	&	3	\\
% 		&	Usability	&		&	3	&	5	\\
% 		&	Portability	&		&	3	&	4	\\
% 		&	Flexibility/Exploitability	&		&	3	&	3	\\
% 		&	Code Quality	&		&	13	&	4	\\
% 		&	Longevity	&		&	7	&	3	\\
% 		&	Coding practices	&		&	4	&	3.5	\\
% 		&	Maintainability	&		&	3	&	4	\\
% 		&	Existence of benchmark/test	&		&	4	&	3.5	\\
% 		&	Update/Upgrade/Add-ons/Plugin	&		&	3	&	4	\\
% 		&	Development process	&		&	3	&	3	\\
% 		&	As-is utility/Quality in use/External quality	&		&	5	&	4	\\
% 		&	Architecture	&		&	5	&	3	\\
% \multicolumn{2}{|l}{	Risk (Perceived risks)	}		&		&	7	&	4.5	\\
% % 		&	Perceived lack of confidentiality	&		&	5	&	1	\\
% 		&	Perceived lack of integrity	&		&	5	&	3	\\
% 		&	Perceived high availability	&		&	5	&	4	\\
% 		&	Perceived high structural assurance	&		&	5	&	2	\\
% 		&	Strategic risks	&		&	5	&	3	\\
% % 		&	Operational risks	&		&	5	&	1	\\
% 		&	Financial risks	&		&	5	&	2	\\
% 		&	Hazard risks	&		&	5	&	4	\\
% \multicolumn{2}{|l}{	Trustworthiness	}		&		&	6	&	4	\\
% 		&	Component	&		&	4	&	3.5	\\	
% 		&	Architecture	&		&	4	&	3	\\	
% 		&	System	&		&	4	&	3.5	\\	
% 		&	OSS provider reputation	&		&	4	&	3.5	\\	
% 		&	Collaboration with other product	&		&	4	&	2.5	\\	
% 		\hline
% \end{tabular}
% \end{table}
\begin{table}
\caption{High-level Factors considered during the adoption of OSS}
\label{tab:interviewees-portals-factors}
\centering
\scriptsize
\adjustbox{center}{
% \begin{tabular}{p{2.5cm}|p{1.1cm}|p{1.5cm}|p{4cm}|}
\begin{tabular}{|ll|p{0.2cm}|c|c|} \hline

\multicolumn{4}{|l|}{	\textbf{RQ1}	} &	 \textbf{RQ2}	%& %\multicolumn{2}{l|}{	 \textbf{RQ3}}
\\ \hline
\multicolumn{2}{|l|}{	Factor	}		&			\#	&	Median	&			\#Measures	%&	Source	&	\%	
\\	 \hline
\multicolumn{2}{|l|}{	Community Support and Adoption	}		&			10	&	4.5	&				%&		&		
\\	  %\hline
		&	Popularity	&			9	&	3	&			4	%&	%R	&	100\%	
		\\	
																			
																			
																			
																			
																			
		&	Community reputation	&			11	&	3	&			3	\\%&	I+\#	&	0.33\%	\\	
																			
																			
																			
																			
																			
																			
		&	Community size	&			13	&	3	&			5	\\%&	R+\#	&	100\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Communication	&			6	&	3.5	&			5	\\%&	I+\#, Q+\#	&	60\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Involvement	&			9	&	3	&			1	\\%&		&	0\%	\\	
																			
																			
																			
																			
		&	Sustainability	&			11	&	3	&			1	\\%&	I+\#	&	100\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Product Team	&			5	&	3	&			2	\\%&	R+\#	&	100\%	\\	
																			
																			
																			
																			
		&	Responsiveness	&			1	&	5	&			1	\\%&	I+\#	&	100\%	\\	
																			
																			
																			
																	
																			
																			
																			
																			
																			
																			
																			  \hline
\multicolumn{2}{|l|}{	Documentation	}		&			14	&	4	&			\\%	&		&		\\	  \hline
		&	Usage documentation	&			4	&	4	&			5	\\%&	R\#, F+	&	100\%	\\	
																			
																			
																			
																			
																			
															
																			
		&	Software requirements	&			11	&	3	&			1	\\%&		&	0\%	\\	
																			
		&	Hardware requirements	&			8	&	3.5	&			1	\\%&		&	0\%	\\	
																			
		&	Software Quality Documentation	&			5	&	3	&			3	\\%&		&	0\%	\\	
																			
																			
																			  \hline
\multicolumn{2}{|l|}{	License	}		&			21	&	4	&			7	\\%&	R	&	14\%	\\	  
\hline
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			 
\multicolumn{2}{|l|}{	Operational SW Characteristics	}		&			6	&	4	&		\\%		&		&		\\	  
%\hline
		&	Trialability	&			5	&	3	&			2	\\%&		&	0\%	\\	
																			
																			
		&	Independence from other SW	&			11	&	3	&			4	\\%&		&	0\%	\\	
																			
																			
																			
																			
		&	Development language	&			5	&	4	&			3	\\%&	R	&	33\%	\\	
																			
																			
																			
		&	Portability	&			1	&	4	&			1	\\%&		&	0\%	\\	
																			
		&	Standard compliance	&			5	&	4	&			0	\\%&		&		\\	
																			
																			
		&	Testability	&			6	&	3.5	&			0	\\%&		&		\\	
																			
																			
																			
																			
																			
																			  \hline
\multicolumn{2}{|l|}{	Maturity	}		&			6	&	3.5	&			11	\\%&	R+\#	&	63\%	\\	  
\hline
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
\multicolumn{2}{|l|}{	Quality	}		&			6	&	3.5	&				\\%&		&		\\	  \hline
																			
		&	Reliability	&			3	&	4	&			6	\\%&	I+\#	&	16\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
		&	Performances	&			4	&	4.5	&			1	\\%&		&	0\%	\\	
																			
																			
																			
																			
																			
																			
		&	Security	&			15	&	4	&			6	\\%&	R+\#, Q+\#, F+\#, S+	&	83\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Modularity	&			3	&	3	&			1	\\%&		&	0\%	\\	
																			
																			
																			
																			
																			
																			
																			
		&	Portability	&			3	&	4	&			2	\\%&		&	0\%	\\	
																			
																			
																			
		&	Flexibility/Exploitability	&			3	&	3	&			3	\\%&		&	0\%	\\	
																			
																			
																			
																			
		&	Code Quality	&			13	&	4	&			6	\\%&		&	16\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Coding conventions	&			9	&	3	&			0	\\%&		&		\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Maintainability	&			3	&	4	&			0	\\%&		&		\\	
																			
		&	Testability	&			2	&	4	&			0	\\%&		&		\\	
		&	Existence of benchmark/test	&			4	&	3.5	&			4	\\%&		&	25\%	\\	
																			
																			
																			
																			
																			
		&	Changeability	&			2	&	3.5	&			0	\\%&		&		\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Update/Upgrade/Add-ons/Plugin	&			3	&	4	&			1	\\%&		&	0\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	Architectural quality	&			5	&	3	&			0	\\%&		&		\\	
																			
																			
																			
																			
																			
																			  \hline
\multicolumn{2}{|l|}{	Risk (Perceived risks)	}		&			7	&	4.5	&				\\%&		&		\\	  
%\hline
		&	Perceived lack of confidentiality	&			5	&	1	&			0	\\%&		&		\\	
		&	Perceived lack of integrity	&			5	&	3	&			0	\\%&		&		\\	
		&	Perceived high availability	&			5	&	4	&			3	\\%&		&	0\%	\\	
																			
																			
																			
		&	Perceived high structural assurance	&			5	&	2	&			0	\\%&		&		\\	
																			
		&	Strategic risks	&			5	&	3	&			0	\\%&		&		\\	
		&	Operational risks	&			5	&	1	&			1	\\%&		&	0\%	\\	
																			
		&	Financial risks	&			5	&	2	&			0	\\%&		&		\\	
		&	Hazard risks	&			5	&	4	&			5	\\%&		&	0\%	\\	
																			
																			
																			
																			
																			
																			
																			  \hline
\multicolumn{2}{|l|}{	Trustworthiness	}		&			6	&	4	&				\\%&		&		\\	  \hline
		&	Component	&			4	&	3.5	&			3	\\%&		&	0\%	\\	
																			
																			
																			
																			
		&	Architecture	&			4	&	3	&			2	\\%&		&	0\%	\\	
																			
																			
																			
		&	System	&			4	&	3.5	&			3	\\%&		&	0\%	\\	
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
																			
		&	OSS provider reputation	&			4	&	3.5	&			0	\\%&		&		\\	
																			
		&	Collaboration with other product	&			4	&	2.5	&			3	\\%&		&	0\%	\\	
																			
																			
																			
																			
																			
																			
																	
																			
																			
																			
																			
		&	Assessment results from 3rd parties	&			2	&	3.75	&			0	\\%&		&		\\	
																			
																			
																			
																			
																			
																			
																			
																			 \hline
\end{tabular}
}
\end{table}
\subsection{RQ2: Measures used by practitioners to evaluate factors during OSS selection}

When we asked practitioners to report the measures they use to evaluate the factors they mentioned in RQ1, and to rank their usefulness, practitioners mentioned 110 different measures.

The complete list of measures reported for each factor is reported in Appendix A. 

In Table~\ref{tab:interviewees-portals-factors} (Column RQ2 - \#Measures we report the count of measures considered as useful by practitioners (likert scale $\geq$ 3, where 0 means ''This measure is useless to evaluate this factor'' and 5 means that the measure is extremely useful). 
% \todo[inline]{This paragraph is a bit unclear. Does the number mean the number of measures/metrics to evaluate the corresponding factor or sub-factor?} 
 
Surprisingly, the factor where practitioners provided the highest number of measures to assess it, is \textit{Maturity}, which has been mentioned only 6 times compared to the \textit{License}, mentioned 21 times,  where practitioners provided 7 measures instead. This indicates a wide variety of interpretations on  \textit{Maturity}, and practitioners use different measures to evaluate this factor. The careful reader can also observe that for some factors considered as relevant in RQ1 such as \textit{Perceived risks}, no measures have been mentioned. This result proves that in some cases, some of the most important factors in an OSS can not be objectively measured and the interviewees do not know how to retrieve such information appropriately. 


\subsection{RQ3: Sources of information and portals used to asses  OSS}
Our interviewees mentioned 9 different source of information and portals they commonly consider when they select OSS.

% \subsubsection{RQ3.1: Sources of Information adopted to evaluate OSS}
In Table~\ref{tab:SoI} we list the sources of information adopted by the practitioners to evaluate OSS, together with the number of participants who mentioned it (columns \# and \% of mentions). To increase the readability, we grouped the source of information in five main categories: \textit{version control systems}, \textit{issue tracking systems}, \textit{Question and Answer portals} (Q\&A), \textit{forum and blogs} and \textit{security} related platforms. 

The 5 most reported sources of information are GitHub (and GitHub Issue tracker), StackOverflow, Reddit, and NIST Security Vulnerability (NVD) with respectively: 23, 19, 12, 12 and 14 mentions. \rt{} All of these are mentioned from more than 20\% of the interviewees and are therefore those which prove to be the most useful when retrieving information related to OSS. Other platforms such as Bitbucket or Jira were rarely mentioned. 

% In addiction to these, we also identified:
% \begin{itemize}
% \begin{itemize}
%     \item OpenHub\footnote{OpenHub: \url{https://www.openhub.net}}
%     %\item NIST Security vulnerability\footnote{NIST Security vulnerability: \url{https://nvd.nist.gov}}
%     \end{itemize} 
% \end{itemize}


% The main sources of information related to version control systems are: Github, GitLab SourgeForge and Bitbucket.

% GitHub\footnote{GitHub: \url{https://github.com}}

% GitLab\footnote{GitLab: \url{https://about.gitlab.com}}

% SourceForge\footnote{SourceForge: \url{https://sourceforge.net}}

% Bitbucket\footnote{Bitbucket: \url{https://bitbucket.org/product/}}
 
% The main issue tracking system is Jira\footnote{Jira: \url{https://www.atlassian.com/software/jira}}.

% The most famous Q\&A portals are: StackOverflow and Reddit.

% StackOverflow\footnote{StackOverflow: \url{https://stackoverflow.com}} and Reddit.

% Reddit\footnote{Reddit: \url{https://www.reddit.com}}

% Forum and blogs used to retreive useful information related to OSS are: Mediuma and Hackernews

% Medium\footnote{Medium: \url{https://medium.com}}

% Hackernews\footnote{Hackernews: \url{https://news.ycombinator.com/news}}

% Some source of information which have been mentioned:  ~\todo[inline]{@Sergio, add link in footnote and add missing ones}
\begin{table}[H]
\caption{The source of information reported by the interviewees (RQ3)}
\label{tab:SoI}
\centering
\scriptsize
% \begin{tabular}{p{2.5cm}|p{1.1cm}|p{1.5cm}|p{4cm}|}
\begin{tabular}{|l|llp{0.1cm}|l|l|} \hline


ID &\multicolumn{2}{l}{	\textbf{Source of Information}	} &		&	\#	&	\textbf{\% of mentions}	\\ \hline
& \multicolumn{2}{l}{	Version Control Systems:	}		&		&		&		\\ \hline
R & 	&	GitHub~\cite{GitHub}	&		&	23	&	100	\\
R &		&	GitLab~\cite{GitLab}	&		&	1	&	4.3	\\
R &		&	SourceForge~\cite{SourceForge}	&		&	1	&	4.3	\\
R &		&	Bitbucket~\cite{Bitbucket}	&		&	1	&	4.3	\\ \hline
& \multicolumn{2}{l}{	Issue Tracking Systems:	}		&		&		&		\\ \hline
I & 	   &   GitHub Issues~\cite{GitHub}	&		&	19	&	82.6	\\
I & 		&	Jira~\cite{Jira}	&		&	1	&	4.3	\\ \hline
& \multicolumn{2}{l}{	Question and Answer Portals:	}		&		&		&		\\ \hline
Q  &         &   StackOverflow~\cite{StackOverflow}	&		&	12	&	51.2	\\
Q & 		&	Reddit~\cite{reddit}	&		&	12	&	51.2	\\ \hline
& \multicolumn{2}{l}{	Forum and Blogs:	}		&		&		&		\\ \hline
F &    &   Medium~\cite{medium} 	&		&	5	&	5	\\
F & 		&	Hackernews~\cite{Hackernews}	&		&	5	&	5	\\
		\hline 
& 		\multicolumn{2}{l}{Security:	}		&		&		&		\\ \hline
S &        &  CVE~\cite{CVE}	&		&	1	&	4.3	\\
S &         &  CVSS~\cite{CVSS}	&		&	2	&	8.7	\\
S &        &  CWE~\cite{CWE} &		&	1	&	4.3	\\
S &  &  NVD~\cite{NVD}	&		&	14&	21.7 	\\
		\hline
\end{tabular}
\end{table}




% \begin{itemize}
%     \item Version control systems:
%     \begin{itemize}
%         \item GitHub\footnote{GitHub: \url{https://github.com}}
%         \item GitLab\footnote{GitLab: \url{https://about.gitlab.com}}
%         \item SourceForge\footnote{SourceForge: \url{https://sourceforge.net}}
%         \item Bitbucket\footnote{Bitbucket: \url{https://bitbucket.org/product/}}
%     \end{itemize}
%     \item Issue tracking systems \begin{itemize}
%         \item GitHub Issues
%         \item Jira\footnote{Jira: \url{https://www.atlassian.com/software/jira}}
%     \end{itemize}
%     \item Question and answers portals
%     \begin{itemize}
%         \item StackOverflow\footnote{StackOverflow: \url{https://stackoverflow.com}}
%         \item Reddit\footnote{Reddit: \url{https://www.reddit.com}}
%     \end{itemize}
%     \item Forums and Blogs 
%     \begin{itemize}
%         \item Medium\footnote{Medium: \url{https://medium.com}}
%         \item Hackernews\footnote{Hackernews: \url{https://news.ycombinator.com/news}}
%     \end{itemize}
% \end{itemize}

% \subsubsection{RQ3.2: Portals adopted to evaluate OSS}
% In Table~\ref{tab:interviewees-portals-info}, we list the portals mentioned by the interviewees.
% \begin{table}[ht!]
% \caption{OSS Source of information and portals mentioned by interviewees}
% \label{tab:interviewees-portals-info}
% \small
% \centering
% % \begin{tabular}{p{2.5cm}|p{1.1cm}|p{1.5cm}|p{4cm}|}
% \begin{tabular}{|l|p{1.3cm}|p{1.4cm}|l|} \hline

% \textbf{Portal}	& 	\textbf{Created on} 	&	\textbf{Last  \quad  activity}	& 	\textbf{Information Stored}	\\ \hline
% \cite{CVE}	CVE	& 	2018	&	2020	& 	Common Vulnerabilities and Exposures \\
% \cite{CVSS}	CVSS	& 	2015	&	2020	& 	Vulnerability Scoring \\
% \cite{CWE}	CWE	& 	2006	&	2020	& 	List of weakness types \\ 
% \cite{NVD}	NVD	& 	2000	&	2020	& 	Vulnerability database \\ 
% \hline
% \end{tabular}
% \end{table}
% Remember to List also the Non mentioned \textbf{NVD} (from literature). As an example Git Archive and SW Heritage are never mentioned. 



\subsection{RQ4: Factors that can be extracted automatically from the portals}

% To answer RQ4, we exploratory investigate the possibility of automatically extracting OSS-projects-related information from popular portals. 

% \todo[inline]{please, add the numbers - Subsection numbers added}
We focused our attention to the four most used sources of information reported in RQ3: GitHub~\cite{GitHub}, StackOverflow~\cite{StackOverflow}, Reddit~\cite{reddit} and the NIST National Vulnerability Database~\cite{NVD}. 
For such purpose, we first identified the  APIs that can be adopted to extract the information needed to measure the factors, and then we extracted the data from the 100k with more stars in GitHub.  

% Some general statistics are shown in Figure \ref{fig:gstats}. 

%recall the list of metrics and sources in the table reported in RQ1
%\todo[inline]{Table with Statistics on factors available per categories (e.g. community 3 out of 5 factors, 50\%)}

The extraction of the information for 100K projects took a total of 5 days for GitHub, 53 days for StackOverflow, 4 days for Reddit and 2 Days for the NIST National Vulnerability Database. 
The long processing time is due to the limit of queries that can be performed on the APIs for different IP addresses. 

% In order to speed-up the computation, we splitted the projects into 5 sets, and we extracted the data from 5 different workstations working on different locations. This separation allowed us to crawl all the information in xxx days.\todo[inline]{The above paragraph could be shifted to Section 3.5 Step 4:...}

Considering the projects extracted (Figure \ref{fig:age}), more than half of these projects (53.3\%) have been active for 2 - 6 years. Around 
12.1\% of these projects are active for one year or less when only 3.9\% of them are active for more than 10 years. Majority of these projects (87.0\%) have less than 500 issues during their life cycle when around 3.4\% of them have more than 1k issues (Figure \ref{fig:issue}). Furthermore, there are 1791 projects being very popular having more than 10k stars when 25.9\% projects having stars ranging from 1k to 10k (Figure \ref{fig:star}) with 46.7\% having less than 500 stars. On the other hand, regarding project size, more than half of them (52.8\%) have lines of code (LOC) ranging from 20k to 500k. 6.1\% projects contain more than 5m LOC when only 0.9\% of them have less than 1k LOC (Figure \ref{fig:loc}). Regarding developing languages, Javascript is the most popular being the primary language of OSS projects (17k projects) with Python and Java at 2nd and 3rd (Figure \ref{fig:pl}). They are the primary languages for 40.9\% of the projects. However, regarding LOC by languages, C language (57.6b) and Javascript (57.2b) rank at the top. Both have almost doubled the amount of C++ language (31.7b) which ranks the 3rd in terms of total LOC (Figure \ref{fig:langloc}). Regarding release numbers, 58.1\% projects do not have any specific release recorded. 37.6\% have less than 50 releases when only the rest 4.3\% have more than 50 releases. 
All the previously mentioned data is always available from GitHub, and queries to the GitHub APIs will always return a valid information, 

Regarding the adopted open source licenses, 23.7\% projects did not specify the licenses they adopt. As for the other projects, MIT, Apache 2.0 and GNU GPL v3.0 are the most popular licenses with 53.2\% projects adopting one of them (Figure \ref{fig:license}). Therein, 13.6\% projects adopted non-mainstream license (identified as 'Other').


We also validate the APIs of Reddit and StackOverflow by finding the amount of discussion threads on each of the 100k OSS projects. As shown in Figure~\ref{fig:rsstats}, 14.5\% projects are generally discussed in Reddit with  only 5.8\% projects having more than 100 posts (Figure \ref{fig:reddit}). On the other hand, 13.0\% projects are discussed (raised technical questions) in StackOverflow (Figure \ref{fig:stack}). Therein, 3.6\% projects have more than 100 questions raised on. In general, such results show that it is hard to find sufficient generic or technical discussion regarding specific OS projects from Reddit and StackOverflow.
%\todo[inline]{In Figure 4 (the distribution of no. of posts in Reddit and Stackoverflow), could we add and show the distribution of projects based on the information from Github e.g. no. of stars, project age, no of releases, etc. That is to say, among the project over 100 posts in Reddit, how many projects have over 1k stars? or how many projects are over 5 year old, or license type, ...? Instead of showing the distribution of projects from one source of information, let us find some connections between the information collected from different sources, if possible.}

\begin{figure}
\centering
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/redditpostsprojects.png}
  \caption{OSS Project Stats by Reddit Post Number}
  \label{fig:reddit}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/stackquestions.png}
  \caption{OSS Project Stats by StackOverflow Questions}
  \label{fig:stack}
\end{subfigure}
\caption{Stats for top 100k Github Projects in Reddit and StackOverflow}
\label{fig:rsstats}
\end{figure}

\begin{figure}
\centering
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/ageyear.png}
  \caption{OSS Project Stats by Age (Years)}
  \label{fig:age}
\end{subfigure}%
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/issue.png}
  \caption{OSS Project Stats by Issues}
  \label{fig:issue}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/stars.png}
  \caption{OSS Project Stats by Stars}
  \label{fig:star}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/locprojects.png}
  \caption{OSS Project Stats by LOC}
  \label{fig:loc}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/primarylanguageTop20.png}
  \caption{OSS Project Stats by Top 20 Primary Languages}
  \label{fig:pl}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/locbylanguageTop20.png}
  \caption{Stats for Top 20 Language by LOC}
  \label{fig:langloc}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/release.png}
  \caption{OSS Project Stats by Releases}
  \label{fig:release}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=\linewidth]{Figures/license_short.png}
  \caption{OSS Project Stats by Licenses}
  \label{fig:license}
\end{subfigure}
\caption{General Stats for Top 100k Github Projects}
\label{fig:gstats}
\end{figure}




Based on the interview results, especially the obtained factors that are considered important by the practitioners (shown in Table~\ref{tab:interviewees-portals-factors}, we further validate whether such factors can be analyzed via the automatically obtained data from the previously mentioned portals with the results shown in Table~\ref{tab:factor_available}.

\begin{table}[]
\caption{Factor Information Availability Stats for Top 100K Projects}
% \todo[inline]{There are also "\#"s in other tables to represent the number, and let us  find another symbol such as "?" to indicate "multiple-queries required" in the column of "Portal".}
\label{tab:factor_available}
\adjustbox{max width=\textwidth}{
%\adjustbox{center}{
\centering
\scriptsize
% \begin{tabular}{p{2.5cm}|p{1.1cm}|p{1.5cm}|p{4cm}|}
\begin{tabular}{|l|l|l|l|} \hline
\textbf{Factor}&\textbf{Portal}&\textbf{\#}&\textbf{\%}\\ \hline
Community Support and Adoption&&&\\

\hspace{2em} Popularity&R&&		\\
\hspace{4em} Number of Watch	&	R	&	100000&	100.00\%		\\
\hspace{4em} Number of Stars	&	R	&	100000&	100.00\%		\\
\hspace{4em} Number of Forks	&	R		&100000	&100.00\%		\\
\hspace{4em} Number of Downloads	&	R	&	42260&	42.26\%		\\

\hspace{2em} Community reputation&I+*&&\\
\hspace{4em} Fast response to issues&I+*	&	100000&	100.00\%	\\

\hspace{2em} Community size	&	R+*	&	&		\\
\hspace{4em}		Number of Contributors	&	R*		&100000	&100.00\%		\\
\hspace{4em}		Number of Subscribers	&	R		&100000	&100.00\%		\\
\hspace{4em}		Community age	&	R+		&100000	&100.00\%		\\
\hspace{4em}		Number of Involved developers per company	&	R+*		&100000	&100.00\%		\\
\hspace{4em}		Number of Independent developers	&	R+*	&	100000&	100.00\%\\
\hspace{2em} Community support	&	R+*, Q+*		&	&	\\
\hspace{4em}		Activeness	&	R+*		&100000&	100.00\%		\\
\hspace{4em}		Responsiveness	&	R+*, Q+*		&14474&	14.47\%		\\
\hspace{2em} Communication	&		I+*, Q+*	&&	\\
\hspace{4em}	Availability of questions/answers	&	I, Q	&	100000&	100.00\%		\\
\hspace{4em} Availability of forum	&	Q	&	14474	&14.47\%		\\
\hspace{4em}		Responsiveness of postings	&	I+*, Q+*	&	14474&	14.47\%		\\
\hspace{4em}		Quality of postings	&	Q+*	&	14474&	14.47\%		\\
\hspace{2em}Sustainability		&	I+*		&		&			\\
\hspace{4em}		Existence of maintainer	&	I+*		&	100000	&	100.00\%		\\
%\hspace{2em} Paid support		&	R+*		&		&			\\
%\hspace{4em}	Availability of official support	&	R+*		&	39499	&	39.50\%		\\

\hspace{2em} Product Team		&	R+*		&		&			\\
\hspace{4em}		Developer quality	&	R+*		&	100000	&	100.00\%		\\
\hspace{4em}		Developer Productivity	&	R+*		&	100000	&	100.00\%		\\
\hspace{2em} Responsiveness	&		I+*		&		&			\\
											
\hspace{4em}		Avg. bug fixing time	&	I+*		&		100000	&	100.00\%			\\
\hspace{4em}		Avg time to implement new issues	&	I+*		&		100000	&	100.00\%			\\

Documentation&&&\\
\hspace{2em} Usage documentation	&		R*, F+		&		&			\\
\hspace{4em}		Availability of updated documentation	&	R*		&	42260	&	42.26\%		\\
\hspace{4em}		Availability of documentation/books/online docs	&	R		&	39499	&	39.50\%		\\
\hspace{4em}		Availability of Tutorial or Examples	&	R		&	39499	&	39.50\%		\\
%\hspace{4em}		Availability of getting started tutorial	&	F+		&		&			\\
%\hspace{4em}		Availability of best practices	&	F+		&		&			\\
License	&	R		&		&			\\
\hspace{2em} License type	&	R		&	76576	&	76.58\%		\\
Operational SW Characteristics	&	R		&		&			\\
\hspace{2em} Development language		&	R		&	93148	&	93.15\%		\\
Maturity	&	R+*		&		&			\\

\hspace{4em} Number of forks	&	R		&	100000	&	100.00\%		\\
\hspace{4em} Release frequency	&	R+*		&	42260	&	42.26\%		\\
\hspace{4em} Number of releases	&	R		&	42260	&	42.26\%		\\
									
\hspace{4em} Age (in Years)	&	R+		&	100000	&	100.00\%		\\
\hspace{4em} Number of commits	&	R		&	100000	&	100.00\%		\\
									
\hspace{4em} Development versions	&	R*		&	42260	&	42.26\%		\\
\hspace{4em} New feature integration	&	R+*		&	42260	&	42.26\%		\\

Quality	&		&		&			\\
\hspace{2em} Reliability &	I+*		&		& \\
\hspace{4em} Average bug age	&	I+*		&	100000	&	100.00\%		\\
\hspace{4em} Avg. bug fixing time	&	I+*		&	100000	&	100.00\%		\\

\hspace{2em}Security		&	R+*, Q+*, S+#		&		&			\\
\hspace{4em}	Number security vulnerabilities	&	S		&12838 &	12.84\%			\\
\hspace{4em}	Number of Vulnerabilities reported on the NVD portal	&	S		&	12838	&	12.84\%		\\

\hspace{4em}	Vulnerability Resolving time	&	R+#, S+		&	12838	&	12.84\%		\\
\hspace{4em}	Community concern towards security	&	R+*, Q+*, S+*		&	12838	&	12.84\%		\\
\hspace{4em}	Vulnerability impact	&	S		&	12838	&	12.84\%		\\
\hspace{2em} Code Quality &R&&\\
\hspace{4em} Code size	&	R		&	100000	&	100.00\%		\\
Trustworthiness&R+*&&\\
\hspace{4em} Consistent release updates pace	&	R+*		&	42260	&	42.26\%		\\
\hline
\end{tabular}
}
\begin{tablenotes}
    \centering
    \tiny
    \item\textit{Repository(R), Issue Tracker(I), Questions and Answer portals(Q), Forum \& Blogs(F), Security(S)}
    \item\textit{Calculation Required(+), Multi-queries Required(*)}
\end{tablenotes}
\end{table}

According to the investigation on automatic OSS data extraction on the top 100k OSS projects on Github via the APIs of the five public portals, we find that the majority of the measures \rf{mentioned by our interviewees (RQ3)},  towards the \textit{Community Support and Adoption} factor can be automatically done via data extractions from such APIs. To be noted, regarding \textit{Communication}, the question and answer sources (i.e., StackOverflow) contain information on limited number of OSS projects, which limits the availability towards the evaluation on such category. In addition, we also find, despite the availability of automatic data extraction and measuring via APIs, many of the measures require further calculation and learning, as well as multiple queries to obtain. For example, in order to measure the \textit{Number of Independent Developers}, we must get the list of contributors of a particular project via multiple queries first (max items per page for Github API is 100), and check the ``Independentness'' of each contributor via further investigating his/her organization status. Thus, such process shall be, to some extent, time-consuming, when the limit rate of the API usage shall be also taken into account. 

Another category can be automatically measured is \textit{License}, as shown in the data, 76.6\% of the projects contain specific License information. On the other hand, for the other categories, automatic data extraction and full-grained evaluation is hindered by the limited availability of the according data, as only very limited percentage of the measures can be automatically done via data extraction (shown in Table \ref{tab:interviewees-portals-factors}). And amongst these categories, the evaluation of \textit{Maturity} category depends on the availability of the release data from repository dataset, when for the obtained 100k projects only 42.2\% provide such information. Measuring the availability of \textit{Documentation} shall also depend on the information extracted from project description and homepage, while only around 40\% of projects provide those. 
%\todo{add numbers for security}
As for the security vulnerability evaluation, the NVD Dataset provide information for 12838 projects (12.8\%). However, it is not clear if the projects not reported in NVD do not contain security vulnerabilities at all, or simply are not indexed by the NVD dataset. However, it is important to note that the NVD performs analysis on CVEs published to the CVE Dictionary. Every CVE has a CVE ID which is used by cybersecurity product/service vendors and researchers for identifying vulnerabilities and for cross-linking with other repositories that also use the CVE ID. However, it is possible that some security vulnerabilities are not publicly reported with assigned CVE IDs.


%, we find that the factors related to \textit{Community Support and Adoption} are relatively easy to be extracted. Therein, three out of the seven factors (\textit{Popularity}, \textit{Community Reputation} and \textit{Communication}) can be measured by, for example, the number of stars, number of questions in StackOverflow and number of posts in Reddit, etc. The other four factors can also be acquired but need further analysis or/and multiple queries. In addition, \textit{License} information can also be directly obtained from Github via APIs. However, the majority of factors in other categories are limitedly available through automatic data extraction. For example, the availability of the documentation can be analyzed by mining the the description of the project on Github; however, the other related information, e.g., requirements, road maps, etc. are not accessible. \textit{Risks}, \textit{maturity} and \textit{trustworthiness} are also hard to measure based on the accessible and acquirable information from public portals, but require complex evaluation process. Regarding \textit{Quality} category, only 1/4 the factors can be measured via data automation, but also requires multiple queries for contributor information and further learning to provide reasonable judgement.



==> Sections/OLD_Background.tex <==
\todo[inline]{Summary of the EUROMICRO literature Review}

This work extends systematic literature review on the OSS evaluation, selection, and adoption published in the 46th Euromicro Conference on Software Engineering and Advanced Applications \cite{Lenarduzzi2020SEAA}. Our previous work compares the existing OSS adoption and selection models, and summarizes the main factors that influence such activities. It covers the 262 studies regarding OSS selection models published by December 2019, which can be used for future investigations into OSS adoption models. Therein, 60 studies are selected, including 20 surveys, 5 lesson learned on OSS adoption motivation and 35 evaluation models reports. Such synthesis of the existing models via SLR reflects the state of the art in the OSS selection and adoption domain. It presents the specification on the proposed OSS evaluation, selection and adoption models with their scopes, building methods and working approach, as well as the enumeration on the common factors considered in such process.

Among the selected 60 studies, their scopes vary greatly with adoption and evaluation being the most common. Meanwhile, community and source code analysis are the unique aspects of evaluating OSS compared to closed source software. Within the proposed 35 models, 21 (60\%) are built via case study, with 5 via interview, 5 via experience and the other 4 via the combination of interview and case study. All proposed models provide either checklist (13 models) or measurement (8 models) or both (14 models) as their working approaches. On the other hand, regarding the studies with surveys and lesson learned, the majority (13) target at adoption motivation identification with the remainders on other scopes. Furthermore, 12 tools are introduced in 22 of the given studies; however, only two out of the 12 are properly maintained.

Regarding the common factors of OSS selection and adoption, eight main categories are elicited, including, \textit{Community and Adoption}, \textit{Development
process}, \textit{Economic}, \textit{Functionality}, \textit{Licence}, \textit{Operational
software characteristics}, \textit{Quality}, \textit{Support and Service}. For each category, sub-factors or metrics are reported. The statistical results, based on the amount of mentioning by different primary studies for each category and sub-factor, show that not all factors are considered equally important according to evaluation models and to surveys and lessons learned. For example, factor \textit{cost} is considered much more important by the surveys than by the models when, on the contrary, the importance of factor \textit{maturity} is seen oppositely. Furthermore, certain factors are considered important by both groups, such as, \textit{Support and Service}, \textit{Code Quality}, \textit{Reliability}, etc. 

In sum, our preceding work presents an overview on the status of OSS selection, evaluation and adoption models in the last two decades, as well as the common factors considered for such process. The contribution shall directly benefit OSS producers by enhancing the likelihood of their products being selected due to their awareness of the required evaluation criteria. It also fulfills the needs of OSS practitioners towards the evaluation of their products in terms of the important factors, especially the overlooked but critical ones.

\todo[inline]{Summary of the extension/Contribution}

Building on such contribution, our preceding work can be still largely improved and more effectively applied towards guiding the OSS selection, evaluation and adoption practices in many ways. Therefore, the contribution of this extension work shall focus on the following aspects. 

==> archived_text.tex <==
\section*{Appendix A: The Selected Sources} 
\label{The Selected Papers}
{\small
  \begin{enumerate}[labelindent=-5pt,label={[S}{\arabic*]}]


% Start copy-paste sources list

\item \label{mezzelira20-2} 	Luca Mezzalira.	"Building Micro-Frontends"  	\\https://www.buildingmicrofrontends.com/,  	2020.  Accessed:2020-05-17
\item \label{Biondic19} 	Denis Biondic. "Building UIs in DevOps / microservices environment part 2— micro-frontends and composite UIs."\\
https://blog.coffeeapplied.com/building-uis-in-devops-microservices-environment-part-2-micro-frontends-and-composite-uis-ab3d4ac394e, 2019.  Accessed:2020-05-17
\item \label{KycPragmatics18} 	Łukasz Kyć	"Independent micro frontends with Single SPA library."  \\	https://blog.pragmatists.com/independent-micro-frontends-with-single-spa-library-a829012dc5be,  	2018.  Accessed:2020-05-17
\item \label{ChauhanSoftobiz19} 	Parijat Chauhan	"Micro Frontend: Extending Microservices to Client-side Development."  	https://www.softobiz.com/micro-frontend-extending-microservices-to-client-side-development/,  	2019.  Accessed:2020-05-17
\item \label{CoyierCssTricks19} 	Chris Coyier	"Micro Frontends." \\
https://css-tricks.com/micro-frontends/,  	2019.  Accessed:2020-05-17
\item \label{JohnsonMedium18} 	Benjamin Johnson	"Exploring micro-frontends."  \\	https://medium.com/@benjamin.d.johnson/exploring-micro-frontends-87a120b3f71c,  	2018.  Accessed:2020-05-17
\item \label{FeatherBuzzfeed19} 	Ian Feather	"Micro Frontends at BuzzFeed." \\  	https://tech.buzzfeed.com/micro-frontends-at-buzzfeed-b8754b31d178,  	2019.  Accessed:2020-05-17
\item \label{GeersMfe19} 	Michael Geers	"Micro Frontends: extending the mircroservice idea to frontend development." \\  	https://micro-frontends.org/,  	2019.  Accessed:2020-05-17
\item \label{HuangDev19} 	Phodal Huang	"Micro-frontend Architecture in Action with six ways."  \\	https://dev.to/phodal/micro-frontend-architecture-in-action-4n60,  	2019.  \\Accessed:2020-05-17
\item \label{KBallZendev19} 	Kevin Ball	"Microfrontends: the good, the bad, and the ugly."  \\	https://zendev.com/2019/06/17/microfrontends-good-bad-ugly.html,  	2019.  \\Accessed:2020-05-17
\item \label{kothariPackt17} 	Amit Kothari	"What is micro frontend?."\\  	https://hub.packtpub.com/what-micro-frontend/,  	2017.  Accessed:2020-05-17
\item \label{MartinFowler19} 	Cam Jackson	"Micro Frontends."\\  	https://martinfowler.com/articles/micro-frontends.html,  	2019.  Accessed:2020-05-17
\item \label{mezzelira19} 	Luca Mezzalira	"Micro-frontends decision framework."  \\	https://lucamezzalira.com/2019/12/22/micro-frontends-decisions-framework/,  	2019.  Accessed:2020-05-17
\item \label{MoralesMedium18} 	Emmanuel Morales	"Micro Front-Ends: Introduction."  \\	https://medium.embengineering.com/micro-front-ends-76171c02ab17,  	2018.  Accessed:2020-05-17
\item \label{MotamediRangle19} 	Ehsan Motamedi	"Five Things to Consider Before Choosing Micro Frontends."  	https://rangle.io/blog/five-things-to-consider-before-choosing-micro-frontends/,  	2019.  Accessed:2020-05-17
\item \label{MyersToptal} 	Bob Myers	"The Strengths and Benefits of Micro Frontends."\\  	https://www.toptal.com/front-end/micro-frontends-strengths-benefits  \\Accessed:2020-05-17
\item \label{PoolaSogeti19} 	Manjuanath Poola	"Micro Frontend Architecture."  	https://labs.sogeti.com/micro-frontend-architecture/,  	2019.  Accessed:2020-05-17
\item \label{BrookSmartPate18} 	Paul Brook	"Microservice Front-end - A Modern Approach to the Division of the front."  	https://www.smartspate.com/microservice-front-end/,  	2018.  Accessed:2020-05-17
\item \label{xenonstack18} 	-	"Micro Frontend Architecture and Best Practices."\\  	https://www.xenonstack.com/insights/what-is-micro-frontend/,  	2018.  Accessed:2020-05-17
\item \label{ZaferHackernoon19} 	Öner Zafer	"Understanding Micro Frontends."\\  	https://hackernoon.com/understanding-micro-frontends-b1c11585a297,  	2019.  Accessed:2020-05-17
\item \label{Nitin19} 	Nitin Jain	"Micro Frontend Curry."\\  	https://levelup.gitconnected.com/micro-frontend-curry-506b98a4cfc0,  	2019. \\ Accessed:2020-05-17
\item \label{Kjartan19} 	Kjartan Rekdal Müller	"Easy Micro-Frontends. "\\ 	https://itnext.io/prototyping-micro-frontends-d03397c5f770,  	2019.  Accessed:2020-05-17
\item \label{xteam17} 	Juan E. Jimenez	"A take on Micro-frontends. "\\ 	https://x-team.com/blog/micro-frontend/,  	2017.  Accessed:2020-05-17
\item \label{AgileChamps17} 	-	"Microservices to Micro-Frontends."\\  	http://www.agilechamps.com/microservices-to-micro-frontends/,  	2017.  Accessed:2020-05-17
\item \label{Altkom18} 	Roberto Witkowski	"UI in Microservices World – Micro Frontends pattern and Web Components."\\  	https://altkomsoftware.pl/en/blog/ui-in-microservices-world/,  	2018.  Accessed:2020-05-17
\item \label{GeersBook20} 	Michael Geers	"Micro Frontends in Action. "\\ 	https://www.manning.com/books/micro-frontends-in-action,  	2020.  \\Accessed:2020-05-17
\item \label{Kumar19} 	Ajay Kumar	"Micro Frontends Architecture."\\	https://www.amazon.com/Micro-Frontends-Architecture-Introduction-Techniques/dp/1097927989,  	2019.  Accessed:2020-05-17
\item \label{SoderlundMedium17} 	Tom Söderlund	"Micro frontends—a microservice approach to front-end web development."\\  	https://medium.com/@tomsoderlund/micro-frontends-a-microservice-approach-to-front-end-web-development-f325ebdadc16,  	2017.  Accessed:2020-05-17
\item \label{HackerNews19} 	"Micro Frontends."  \\	https://news.ycombinator.com/item?id=20148308,  	2019.  Accessed:2020-05-17
\item \label{Luigi18} 	"The Enterprise-Ready Micro Frontend Framework."\\  	https://luigi-project.io/about,  	2018.  Accessed:2020-05-17
\item \label{Spa15} "Single-spa: A javascript router for front-end microservices."\\  	https://single-spa.js.org/,  	2015.  Accessed:2020-05-17
\item \label{Slideshare16} 	Luiz Mineiro "The frontend taboo."\\  	https://www.slideshare.net/lmineiro/the-frontend-taboo-a-story-of-full-stack-microservices,  	2016.  Accessed:2020-05-17
\item \label{Smashing19} 	Luca Mezzalira	"Smashing Podcast Episode 6: What Are Micro-Frontends?."\\   Smassing Magazine 	https://www.smashingmagazine.com/2019/12/smashing-podcast-episode-6/,  	2019.  Accessed:2020-05-17
\item \label{case18} 	Gustaf Nilsson Kotte	"Micro Frontends with Gustaf Nilsson Kotte."  \\	https://www.case-podcast.org/22-micro-frontends-with-gustaf-nilsson-kotte,  	2018.  Accessed:2020-05-17
\item \label{Thoughtworks19} 	Thoughtswork podacast	"What's cool about micro frontends." \\	https://thoughtworks.libsyn.com/whats-so-cool-about-micro-frontends,  	2019.  Accessed:2020-05-17
\item \label{thoughtworksRadar16} 	Thoughtworks	"Technology radar: Micro frontends."  \\	https://www.thoughtworks.com/radar/techniques/micro-frontends,  	2016.  \\Accessed:2020-05-17
\item \label{Grijsen19} 	Erik Grijzen	"Micro Frontend Architecture Building an Extensible UI Platform."\\  	https://www.youtube.com/watch?v=9Xo-rGUq-6E,  	2019.  Accessed:2020-05-17
\item \label{Gohen19} 	Liron Cohen	"Micro-frontends: Is it a Silver Bullet?" | React Next 2019. \\ 	https://www.youtube.com/watch?v=asqgKaUMXq0,  	2019.  Accessed:2020-05-17
\item \label{Engel18} 	Elisabeth Engel	"Break Up With Your Frontend Monolith" JSCamp Barcelona 2018.  https://tinyurl.com/y5ksc2fm,  	2018.  Accessed:2020-05-17
\item \label{Mosaic9} 	Zalando	"Project Mosaic | Microservices for the Frontend."  	\\https://www.mosaic9.org/,  	2016.  Accessed:2020-05-17
\item \label{Krishnamurthy19} 	Santhosh Krishnamurthy	"What are Micro Frontends."  IEEE India Info. Vol. 14, No. 4, Oct-Dec 2019	
\item \label{YangLiuSuIOP19} 	Caifang Yang, Chuanchang Liu, Zhiuaun Su	"Research and Application of Micro Frontends." IOP Conference on Materials Science and Engineering. 2019. DOI: 10.1088/1757-899x/490/6/062082\\
\item \label{PavlovEtAl2020} Andrey Pavlenko, Nursultan Askarbekuly, Swati Megha, Manuel Mazzara
"Micro-frontends: application of microservices to web front-ends. "\\ Journal of Internet Services and Information Security (JISIS), volume: 10, number: 2 (May 2020), pp. 49-66 DOI: 10.22667/JISIS.2020.05.31.049
% end copy paste source list
\end{enumerate}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%
% Search engines
%%
@misc{ACMDigital,
  title = {ACM digital Library},
  year = {-},
  howpublished = {\url{IEEEXplore Digital Library}},
  note = {Accessed: 2020-04}
}


@misc{IEEEXplore,
  title = {IEEEXplore Digital Library},
  year = {-},
  howpublished = {\url{http:ieeexplore.ieee.org}},
  note = {Accessed: 2020-04}
}

@misc{ScienceD,
  title = {Science Direct},
  year = {-},
  howpublished = {\url{http:www.sciencedirect.com}},
  note = {Accessed: 2020-04}
}

@misc{Scopus,
  title = {Scopus},
  year = {-},
  howpublished = {\url{https:www.scopus.com}},
  note = {Accessed: 2020-04}
}

@misc{GoogleS,
  title = {Google Scholar},
  year = {-},
  howpublished = {\url{http:scholar.google.com}},
  note = {Accessed: 2020-04}
}

@misc{CiteseerL,
  title = {Citeseer library},
  year = {-},
  howpublished = {\url{http:citeseer.ist.psu.edu}},
  note = {Accessed: 2020-04}
}

@misc{Inspec,
  title = {Inspec},
  year = {-},
  howpublished = {\url{(http:iee.org/Publish/INSPEC/}},
  note = {Accessed: 2020-04}
}

@misc{SpringerL,
  title = {Springer link},
  year = {-},
  howpublished = {\url{(https:link.springer.com/}},
  note = {Accessed: 2020-04}
}

@misc{Ikea,
  title = {Experiences Using Micro Frontends at IKEA},
  year = {2018},
  howpublished = {\url{https://www.infoq.com/news/2018/08/experiences-micro-frontends/}},
  note = {Accessed: 2020-05-29}
}

@misc{Spotify,
  title = {Adopting a Micro-frontends architecture},
  year = {2019},
    howpublished = {\url{https://lucamezzalira.com/2019/04/08/adopting-a-micro-frontends-architecture/}},
    note = {Accessed: 2020-05-29}
}


@misc{Medium,
    title={Medium},
    year = {-},
    howpublished={\url{https://medium.com/}},
    note = {Accessed: 2020-06}
}

@misc{Reddit,
    title={Reddit},
    year = {-},
    howpublished={\url{https://www.reddit.com/}},
    note = {Accessed: 2020-06}
}

@misc{Twitter,
    title={Twitter},
    year = {-},
    howpublished={\url{https://twitter.com/}},
    note = {Accessed: 2020-06}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% AAA
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% BBB
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@ARTICLE{Bosch16a,
author={J. {Bosch}},
journal={IEEE Software},
title={Speed, Data, and Ecosystems: The Future of Software Engineering},
year={2016},
volume={33},
number={1},
pages={82-88},}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% CCC
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% DDD
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% EEE
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% FFF
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% GGG
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In Latex doc, type \cite{ref_id} to add ref to this record. 
% ref_id is of type <Firstauthor><Year><Letter>
% <Firstauthor> = last name of first author, e.g. salminen
% <Year>        = two numbers, e.g. 03
% <Letter>      = 'running number' to distinquish several refs of
%                 one author on a given year, start with a
% use only small case letters and no white spaces, e.g. salminen03a
% Explanations from: http://www.ecst.csuchico.edu/~jacobsd/bib/formats/bibtex.html

%Garousi,Vahid and Felderer,Michael and Mäntylä,Mika,V.
%Guidelines for including grey literature and conducting %multivocal literature reviews in software engineering
@article{Garousi18a,
title = "Guidelines for including grey literature and conducting multivocal literature reviews in software engineering",
journal = "Information and Software Technology",
volume = "106",
pages = "101 - 121",
year = "2019",
issn = "0950-5849",
doi = "https://doi.org/10.1016/j.infsof.2018.09.006",
url = "http://www.sciencedirect.com/science/article/pii/S0950584918301939",
author = "Vahid Garousi and Michael Felderer and Mika V. Mäntylä",
keywords = "Multivocal literature review, Grey literature, Guidelines, Systematic literature review, Systematic mapping study, Literature study, Evidence-based software engineering",
}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% HHH
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% III
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% JJJ
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% KKK
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@book{Khononov19a,
  author = 	 {Khononoc, Vladik},
  title = 	 {What is domain-driven design?},
  journal =  {O’Reilly Media},
  year = 	 {2019},
  volume = 	 {},
  number = 	 {},
  pages = 	 {},
  month = 	 {},
  }

@book{Kumar19a,
  author = 	 {Ajay Kumar},
  title = 	 {Micro Frontends Architecture},
  journal =  {Amazon fulfillment},
  year = 	 {2019},
  volume = 	 {},
  number = 	 {},
  pages = 	 {},
  month = 	 {},
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% LLL
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@inproceedings{Chen18a,
author = {Chen, Lianping},
year = {2018},
month = {03},
pages = {},
title = {Microservices: Architecting for Continuous Delivery and DevOps},
doi = {10.1109/ICSA.2018.00013}
}

@misc{LuigiFramework,
  title = {Luigi project},
  year = {2018},
  howpublished = {\url{https://luigi-project.io/}},
  note = {Accessed: 2020-05-14}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% MMM
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@misc{MooaFramework18,
author = {Huang, Phodal },
title = {Mooa Framework},
year = {2018},
howpublished = {\url{https://github.com/phodal/mooa}},
note = {Accessed: 2020-05-17}
}

@ARTICLE{Menaetal19,
  author={M. {Mena} and A. {Corral} and L. {Iribarne} and J. {Criado}},
  journal={IEEE Access}, 
  title={A Progressive Web Application Based on Microservices Combining Geospatial Data and the Internet of Things}, 
  year={2019},
  volume={7},
  number={},
  pages={104577-104590},}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% NNN
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% OOO
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% PPP
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% RRR
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% SSS
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@misc{SingleSpa,
  title = {Single-SPA framework},
  year = {2015},
  howpublished = {\url{https://single-spa.js.org/}},
  note = {Accessed: 2020-05-14}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% TTT
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@misc{thoughtworksTechRadar,
  title = {Technology radar: micro frontends},
  year={2016},
  howpublished={\url{https://www.thoughtworks.com/radar/techniques/micro-frontends}},
  note={Accessed: 2020.05.14}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% UUU
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% VVV, WWW
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% XXX, YYY, ZZZ
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
@misc{ZalandoMosaic,
  year = {2016},
  title = {Project Mosaic},
  howpublished = {\url{https://www.mosaic9.org/}},
  note = {Accessed: 2020-05-14}
}

@techreport{Kitchenham2007,
  abstract = {The objective of this report is to propose comprehensive guidelines for systematic literature reviews appropriate for software engineering researchers, including PhD students. A systematic literature review is a means of evaluating and interpreting all available research relevant to a particular research question, topic area, or phenomenon of interest. Systematic reviews aim to present a fair evaluation of a research topic by using a trustworthy, rigorous, and auditable methodology. The guidelines presented in this report were derived from three existing guidelines used by medical researchers, two books produced by researchers with social science backgrounds and discussions with researchers from other disciplines who are involved in evidence-based practice. The guidelines have been adapted to reflect the specific problems of software engineering research. The guidelines cover three phases of a systematic literature review: planning the review, conducting the review and reporting the review. They provide a relatively high level description. They do not consider the impact of the research questions on the review procedures, nor do they specify in detail the mechanisms needed to perform meta-analysis. test chapter},
  added-at = {2010-10-18T14:00:32.000+0200},
  at = {2009-01-27 02:42:01},
  author = {Kitchenham, Barbara and Charters, Stuart},
  biburl = {https://www.bibsonomy.org/bibtex/227b256010a48688388374cf83b619b54/msn},
  id = {3955888},
  institution = {Keele University and Durham University Joint Report},
  interhash = {aed0229656ada843d3e3f24e5e5c9eb9},
  intrahash = {27b256010a48688388374cf83b619b54},
  keywords = {research.cs.softeng research.support},
  number = {EBSE 2007-001},
  priority = {2},
  timestamp = {2010-10-18T14:00:32.000+0200},
  title = {Guidelines for performing Systematic Literature Reviews in Software Engineering},
  howpublished = {http://www.dur.ac.uk/ebse/resources/Systematic-reviews-5-8.pdf},
  year = 2007
}

@article{Balalaie2018,
author = {Balalaie, Armin and Heydarnoori, Abbas and Jamshidi, Pooyan and Tamburri, Damian A. and Lynn, Theo},
title = {Microservices migration patterns},
journal = {Software: Practice and Experience},
volume = {48},
number = {11},
pages = {2019-2042},
keywords = {cloud-native architectures, cloud computing, microservices, migration patterns},
doi = {10.1002/spe.2608},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/spe.2608},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/spe.2608},
abstract = {Summary Microservices architectures are becoming the defacto standard for building continuously deployed systems. At the same time, there is a substantial growth in the demand for migrating on-premise legacy applications to the cloud. In this context, organizations tend to migrate their traditional architectures into cloud-native architectures using microservices. This article reports a set of migration and rearchitecting design patterns that we have empirically identified and collected from industrial-scale software migration projects. These migration patterns can help information technology organizations plan their migration projects toward microservices more efficiently and effectively. In addition, the proposed patterns facilitate the definition of migration plans by pattern composition. Qualitative empirical research is used to evaluate the validity of the proposed patterns. Our findings suggest that the proposed patterns are evident in other architectural refactoring and migration projects and strong candidates for effective patterns in system migrations.},
year = {2018}
}


@article{SOLDANI2018,
title = "The pains and gains of microservices: A Systematic grey literature review",
journal = "Journal of Systems and Software",
volume = "146",
pages = "215 - 232",
year = "2018",
issn = "0164-1212",
doi = "https://doi.org/10.1016/j.jss.2018.09.082",
url = "http://www.sciencedirect.com/science/article/pii/S0164121218302139",
author = "Jacopo Soldani and Damian Andrew Tamburri and Willem-Jan {Van Den Heuvel}",
keywords = "Microservices, Microservices design, Microservices development, Microservices operation, Systematic grey literature review, Systematic literature review",
abstract = "The design, development, and operation of microservices are picking up more and more momentum in the IT industry. At the same time, academic work on the topic is at an early stage, and still on the way to distilling the actual “Pains & Gains” of microservices as an architectural style. Having witnessed this gap, we set forth to systematically analyze the industrial grey literature on microservices, to identify the technical/operational pains and gains of the microservice-based architectural style. We conclude by discussing research directions stemming out from our analysis."
}



@article{Yang_2018,
	doi = {10.1088/1757-899x/490/6/062082},
	url = {https://doi.org/10.1088\%2F1757-899x\%2F490\%2F6\%2F062082},
	year = 2019,
	month = {apr},
	publisher = {{IOP} Publishing},
	volume = {490},
	pages = {062082},
	author = {Caifang Yang and Chuanchang Liu and Zhiyuan Su},
	title = {Research and Application of Micro Frontends},
	journal = {{IOP} Conference Series: Materials Science and Engineering},
	abstract = {The content management system is an indispensable part of enterprise information construction. With the rise of the concept of front and rear separation and the maturity of related technologies, it is a better choice to create a multi-functional front-end web application in complex large-sized or medium-sized projects, which sits on top of a microservices-based architecture. As the business grows, the single front end becomes more and more bloated, resulting in a single page application that is not well scaled and deployed, and difficult to maintain. Based on the analysis of above problems, combined with the corresponding front-end technology, this paper applies the microservice concept to the development of front-end and proposes a design scheme of content management system based on micro frontends. Besides, the key issues in practice process, such as micro frontends design concept and implementation methods are described in detail.}
}

@book{groundedTheory,
  added-at = {2008-01-28T14:18:40.000+0100},
  address = {Newbury Park, California},
  author = {Strauss, A. and Corbin, J.},
  biburl = {https://www.bibsonomy.org/bibtex/2027e373b0616861eb56c15a9c34d5cf6/wiljami74},
  description = {Basics of qualitative research: grounded theory procedures and techniques A. Strauss J. Corbin},
  interhash = {3b7714191aef15ecd7a2665ab11f1e0f},
  intrahash = {027e373b0616861eb56c15a9c34d5cf6},
  keywords = {grounded_theory},
  publisher = {Sage Publications},
  timestamp = {2008-01-28T14:18:40.000+0100},
  title = {Basics of Qualitative Research: Grounded Theory Procedures and Techniques},
  year = 1990
}

@ARTICLE{TaibiIEEECloud2017, 
author={D. Taibi and V. Lenarduzzi and C. Pahl}, 
journal={IEEE Cloud Computing}, 
title={Processes, Motivations, and Issues for Migrating to Microservices Architectures: An Empirical Investigation}, 
year={2017}, 
volume={4}, 
number={5}, 
pages={22-32}, 
keywords={software architecture;Web services;microservice architectures;return on investment;nontechnical motivation;technical motivations;scalability motivation;maintainability motivation;migration processes;Companies;Computer architecture;Cloud computing;Scalability;Investment;Maintenance engineering;microservices;cloud native;cloud migration;cloud computing;cloud containers;Docker;service oriented architectures SOA}, 
doi={10.1109/MCC.2017.4250931}, 
ISSN={2325-6095}, 
month={Sep.},}

@ARTICLE{MezzaliraIEEESW2020, 
author={D. Taibi and L.Mezzalira}, 
journal={IEEE Software (Column)}, 
title={Micro-Frontends: Principles, Benefits and Pitfalls}, 
year={2020}, 
note={Under Review}}






@book{MezzaliraBook,
  author = 	 {Mezzalira, Luca},
  title = 	 {Building Micro-Frontends},
  journal =  {O’Reilly Media},
  year = 	 {2021},
  volume = 	 {},
  number = 	 {},
  pages = 	 {},
  month = 	 {April},
  ISBN = {9781492082927}

  }

@misc{Soderlund,
    author = {Söderlund, Tom},
    title = {Micro frontends—a microservice approach to front-end web development},
    howpublished = {https://medium.com/@tomsoderlund/micro-frontends-a-microservice-approach-to-front-end-web-development-f325ebdadc16},
    year = {2017},
}

@misc{GeersMichael,
    author = {Geers, Michael},
    title = {Extending the microservice idea to frontend development},
    note = {https://micro-frontends.org/},
    year ={2020}
}

@misc{Peltonen2020,
author = {Severi Peltonen and Luca Mezzalira and Davide Taibi},
title = {[RAW-DATA] Motivations, Benefits and Issues for adopting Micro-Frontends: A Multivocal Literature Review},
year = {2020},
month = {6},
howpublished = {\url{https://figshare.com/articles/dataset/_RAW-DATA_Motivations_Benefits_and_Issues_for_adopting_Micro-Frontends_A_Multivocal_Literature_Review/12587708}},
doi = {10.6084/m9.figshare.12587708.v1}
}

@misc{AkamaiOracle,
author= {M.Tsimelzon and B.Weihl and J.Chung and D.Frantz and J.Basso and C.Newton and M.Hale and L.Jacobs and C.O'Connell},
year={2001},
howpublished={https://www.w3.org/TR/esi-lang/},
}

@article{Pavlenko2020,
author={Andrey Pavlenko and Nursultan Askarbekuly and Swati Megha, Manuel Mazzara},
year={2020},
journal={Journal of Internet Services and Information Security},
volume = {10},
number = {2},
year = {2020}, 
month = {August}, 
title={Micro-frontends: application of microservices to web front-ends},
howpublished={\url{http://isyou.info/jisis/vol10/no2/jisis-2020-vol10-no2-04.pdf}}
}





@article{EUmobileUsage,
title={Internet use by individuals},
year={2016},
journal={eurostat},
url={https://ec.europa.eu/eurostat/documents/2995521/7771139/9-20122016-BP-EN.pdf},
}

@misc{FruhlingerJamstack,
title={Jamstack: The static website revolution upending web development},
howpublished={https://www.infoworld.com/article/3563829/jamstack-the-static-website-revolution-upending-web-development.html},
note = {Accessed: 2020-08}
}

@misc{DomCSR,
title={Document Object Model (DOM) Level 1 Specificatio},
year={1998},
howpublished={https://www.w3.org/TR/1998/REC-DOM-Level-1-19981001/},
}

@book{MixuSPA,
title={Modern web applications: an overview},
author={Mikito Takada},
year={2013},
howpublished={http://singlepageappbook.com/goal.html},
}

@book{SPA,
author={M. Mikowski and J. Powell},
title={Single Page Web Applications},
year={2013},
publisher = {Manning Publications Company},
}

@misc{w3schools,
title={JavaScript HTML DOM},
howpublished={https://www.w3schools.com/js/js\_htmldom.asp},
note = {Accessed: 2020-09},
year={-}
}


@misc{AngularSPA,
title={Angular},
howpublished={https://angular.io/},
year={-},
note = {Accessed: 2020-09}
}

@misc{ReactSpa,
title={ReactJs},
howpublished={https://reactjs.org/},
note = {Accessed: 2020-09},
year={-},
}

@misc{VueJs,
title={VueJs},
howpublished={https://vuejs.org/},
note = {Accessed: 2020-09},
year={-},
}

@article{jadhavAngular,
title={Single Page Application using AngularJS},
url={http://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.736.4771&rep=rep1&type=pdf},
year={2015},
journal={International Journal of Computer Science and Information Technologies 6.3},
pages={2876-2879}
}

@misc{SpaVsJamstack,
title={Can a SPA be JAMstack?},
howpublished={https://dev.to/shortdiv/can-a-spa-be-jamstack-5gci},
note = {Accessed: 2020-08},
}

@misc{AngularLifeCycle,
title={Hooking into the component lifecycle},
howpublished={https://angular.io/guide/lifecycle-hooks},
year={2020},
note = {Accessed: 2020-08},
}

@misc{VueJsLifeCycle,
title={Instance Lifecycle Hooks},
howpublished={https://vuejs.org/v2/guide/instance.html\#Instance-Lifecycle-Hooks},
year={2020},
note = {Accessed: 2020-08},
}

@misc{ReactJsLifeCycle,
title={State and Lifecycle},
howpublished={https://reactjs.org/docs/state-and-lifecycle.html\#adding-lifecycle-methods-to-a-class},
note = {Accessed: 2020-08},
}

@article{KotteIsomorphic,
author= {Gustaf Nilsson Kotte},
year={2016},
title={6 Reasons Isomorphic Web Apps is not the Silver Bullet You’re Looking For},
url={https://blog.jayway.com/2016/05/23/6-reasons-isomorphic-web-apps-not-silver-bullet-youre-looking/},
note={Accessed: 2020-08}
}

@article{MediumIsomorphic,
author={AirbnbEng},
title={Isomorphic JavaScript: The Future of Web Apps},
year={2013},
url={https://medium.com/airbnb-engineering/isomorphic-javascript-the-future-of-web-apps-10882b7a2ebc},
}


@book{WohlinExperimentation,
  added-at = {2012-11-09T00:00:00.000+0100},
  author = {Wohlin, Claes and Runeson, Per and Höst, Martin and Ohlsson, Magnus C. and Regnell, Björn},
  biburl = {https://www.bibsonomy.org/bibtex/2d11009fb82f65d8cb854966a049dcd08/dblp},
  ee = {http://dx.doi.org/10.1007/978-3-642-29044-2},
  interhash = {1bdbcb69db1906784cbf84acfd08c3f6},
  intrahash = {d11009fb82f65d8cb854966a049dcd08},
  isbn = {978-3-642-29043-5},
  keywords = {dblp},
  pages = {I-XXIII, 1-236},
  publisher = {Springer},
  timestamp = {2012-11-10T11:53:32.000+0100},
  title = {Experimentation in Software Engineering.},
  year = 2012
}

